Farthest points on most Alexandrov surfaces

We study global maxima of distance functions on most Alexandrov surfaces with curvature bounded below, where "most" is used in the sense of Baire categories.

==> Macros.tex <==
% V 2.1
\newcommand{\nc}{\newcommand}
\newcommand{\df}{\def}
\RequirePackage{ifthen}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%racourciss divers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\df\ie#1{{\mbox{{\it i.\hspace{0.06em}e.}\ifthenelse{\equal{#1}{,}}{\hspace{0.06em},}{\ #1}}}}
\df\eg#1{{\mbox{{\it e.\hspace{0.06em}g.}\ifthenelse{\equal{#1}{,}}{\hspace{0.06em},}{\ #1}}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Citations dans Theorem
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\cit}[2][]{\ifthenelse{\equal{#1}{}}{{\rm \cite{#2}}}{{\rm \cite[#1]{#2}}}}

\makeatletter

%%%%%%%%%TURNED-M

\newcommand{\most@textstyle}{\hspace{.07em plus .01 em minus .01em}\rule[-.1pt]{.35pt}{1.63ex}\hspace{-.315 em}\wedge\hspace{-.315 em}\rule[-.1pt]{.35pt}{1.63ex}\hspace{.15em plus .05em minus .05em}}

\newcommand{\most@scriptstyle}{\hspace{.05705em plus .00815 em minus .00815em}\rule[-.1pt]{.33pt}{1.139ex}\hspace{-.07 em}\wedge\hspace{-.07 em}\rule[-.1pt]{.33pt}{1.139ex}\hspace{.12225em plus .04075em minus .04075em}}

\newcommand{\most@scriptscriptstyle}{\hspace{.05075em plus .00725 em minus .00725em}\rule[-.1pt]{.32pt}{0.815ex}\hspace{-.063 em}\wedge\hspace{-.065 em}\rule[-.1pt]{.32pt}{0.815ex}\hspace{.10875em plus .03625em minus .03625em}}

\newcommand{\most}{\mathchoice{\most@textstyle}{\most@textstyle}{\most@scriptstyle}{\most@scriptscriptstyle}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Gestions des {|}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% usage:  \set(: xyz\in XYZ | xyz is something :) 
%
%Note: \set[xx](: ...| ...:) is for backward compatibility, xx is ignored.
%Note: \seti is an alias of \set, still for backward compatibility
%Note: If set are nested, inner sets must be enclosed in braces: {\set(:...|...:)}


\newlength{\Set@LH}
\newlength{\Set@RH}
\newlength{\Set@LD}
\newlength{\Set@RD}
\newlength{\Set@NoPar@W}

\newsavebox{\Set@Box@R}
\newsavebox{\Set@Box@L}

\newcommand{\Set@@}[3]{%#3=math style
\sbox{\Set@Box@L}{\ensuremath{#3#1}}
\sbox{\Set@Box@R}{\ensuremath{#3#2}}
\settoheight{\Set@LH}{\usebox{\Set@Box@L}}
\settodepth {\Set@LD}{\usebox{\Set@Box@L}}
\settoheight{\Set@RH}{\usebox{\Set@Box@R}}
\settodepth {\Set@RD}{\usebox{\Set@Box@R}}
\addtolength{\Set@LH}{\Set@LD}
\addtolength{\Set@RH}{\Set@RD}
{\def\mt{\rule[-\Set@LD]{0pt}{\Set@LH}\rule[-\Set@RD]{0pt}{\Set@RH}}
\settowidth{\Set@NoPar@W}{\ensuremath{#3\left.\mt\right.}}
\left\{\usebox{\Set@Box@L}\mt\right.\hspace{-.3\Set@NoPar@W}\left\vert\usebox{\Set@Box@R}\mt\right\}}
}


\def\Set@Smile(:#1|#2:){\mathchoice
{\Set@@{#1}{#2}{\displaystyle}}
{\Set@@{#1}{#2}{\textstyle}}
{\Set@@{#1}{#2}{\scriptstyle}}
{\Set@@{#1}{#2}{\scriptscriptstyle}}
}

\newcommand{\set}[1][]{\Set@Smile}
\newcommand{\seti}{\set}




\makeatother


